Turing Kernelization for Finding Long Paths in Graph Classes Excluding a Topological Minor

The notion of Turing kernelization investigates whether a polynomial-time algorithm can solve an NP-hard problem, when it is aided by an oracle that can be queried for the answers to bounded-size subproblems. One of the main open problems in this direction is whether k-Path admits a polynomial Turing kernel: can a polynomial-time algorithm determine whether an undirected graph has a simple path of length k, using an oracle that answers queries of size poly(k)? We show this can be done when the input graph avoids a fixed graph H as a topological minor, thereby significantly generalizing an earlier result for bounded-degree and $K_{3,t}$-minor-free graphs. Moreover, we show that k-Path even admits a polynomial Turing kernel when the input graph is not H-topological-minor-free itself, but contains a known vertex modulator of size bounded polynomially in the parameter, whose deletion makes it so. To obtain our results, we build on the graph minors decomposition to show that any H-topological-minor-free graph that does not contain a k-path, has a separation that can safely be reduced after communication with the oracle.

==> tw-modulator.tex <==
In this section we focus on the parameterization of the
\kPath{} problem not only by the desired path length $k$,
but also by a size of a given modulator to graphs of constant treewidth.
We prove Theorem~\ref{thm:eta-main}; that is, let us fix an integer constant $\eta > 0$.
Recall that a set $M \subseteq V(G)$ is a \emph{$\eta$-treewidth modulator}
if $G-M$ has treewidth at most $\eta$.
We assume that, apart from the input \kPath{} instance $(G,k)$ we are given
also an $\eta$-treewidth modulator $M$ of size $\ell := |M|$, and we study
joint parameterization by $k$ and $\ell$.
As in the previous case, we actually reduce to the \kLinkage{} problem, 
   showing the following.

\begin{theorem}\label{thm:eta-main2}
For every fixed integer
$\eta > 0$, one can solve in polynomial time a given \kPath{} instance $(G,k)$,
given access to an $\eta$-treewidth modulator $M$ of size $\ell$
and an oracle that solves the \kLinkage{} problem for instances $(G',k', (R_i)_{i=1}^r)$
with $G'$ being a subgraph of $G$, $r, k' \leq k$, and $|V(G')| = \Oh(k^4 \ell^{4\eta+6})$.
\end{theorem}

In the remainder of this section we prove Theorem~\ref{thm:eta-main2}.

\paragraph{Marking.}
We start with a somewhat standard marking process.
For an integer $0 \leq k' \leq k-2$ and two vertices $u, v \in M$, define a
\emph{$(u,v,k')$-path} in $G$ as a (simple) path with $k'+2$ vertices: two endpoints $u$ and $v$
and exactly $k'$ internal vertices, all in $G-M$.
Note that a $(u,v,0)$-path is a path consisting of an edge $uv$.
Similarly, for $0 \leq k' \leq k-1$ and a vertex $u \in M$, a $(u,k')$-path
in $G$ is a path with $k'+1$ vertices: one endpoint being $u$ and all other vertices
in $G-M$.

For every $0 \leq k' \leq k-2$ and every $u,v\in M$, we compute an inclusion-wise maximal
family $\mathcal{P}_{u,v,k'}^0$ of internally vertex-disjoint $(u,v,k')$-paths.
Note that, as $G-M$ has constant treewidth, this can be done in polynomial time by standard
dynamic programming methods. Similarly, for every $0 \leq k' \leq k-1$ and $u \in M$
we compute an inclusion-wise maximal family $\mathcal{P}_{u,k'}^0$ of internally
vertex-disjoint $(u,k')$-paths. 
We define $\mathcal{P}_{u,v,k'}$ to be a subfamily of $k+1$ arbitrarily chosen 
paths from $\mathcal{P}_{u,v,k'}^0$, or let $\mathcal{P}_{u,v,k'} = \mathcal{P}_{u,v,k'}^0$
if $|\mathcal{P}_{u,v,k'}| < k+1$. We define $\mathcal{P}_{u,k'}$ similarly.

Let $A_1$ be the set of all vertices of $G-M$ that lie on some path
in any of the sets $\mathcal{P}_{u,v,k'}$ or $\mathcal{P}_{u,k'}$ ($u,v\in M$, $k'\leq k$). Note that,
   as we picked at most $k+1$ paths to the families 
   $\mathcal{P}_{u,v,k'}$ and $\mathcal{P}_{u,k'}$, we have
$$|A_1| < (k+1) \cdot k \cdot \ell^2.$$

Fix a tree decomposition $(T,\X)$ of $G-M$ of width at most $\eta$;
since $\eta$ is a constant, such a decomposition can be computed in linear time
using the algorithm of Bodlaender~\cite{Bodlaender96}.
By possibly duplicating some nodes, we can assume that every node of $T$ has at most two
children.

For every $x \in A_1$, pick one node $t(x) \in V(T)$ such that $x \in \X(t(x))$.
Let $B_1 = \{t(x) \mid x \in A_1\}$.
Let $B_2 \subseteq V(T)$ consist of all of $B_1$, the root of $T$, and the lowest
common ancestor of every pair $(t_1,t_2) \in B_1 \times B_1$.
Let $A_2 = \X(B_2)$.
It is folklore that $|B_2| \leq 2|B_1|$, hence:
\begin{align*}
|B_2| &\leq 2k(k+1)\ell^2,\\
|A_2| &\leq 2(\eta+1)k(k+1)\ell^2.
\end{align*}

We say that two edges $e_1,e_2 \in E(T)$ are \emph{connected} if
there is a path in $T$ containing $e_1$ and $e_2$ that does not contain any node
of $B_2$ as an internal vertex. Since $T$ is a tree, the notion of being connected is an equivalence
relation. A \emph{component} is an equivalence class in this relation.

Fix a component $C \subseteq E(T)$.
As $B_2$ is closed under taking lowest common ancestors of nodes,
we have that $V(C)$ contains at most two nodes of $B_2$. Furthermore, as $(V(C),C)$
is a subtree of $T$ and $B_2$ contains the root of $T$, the topmost node of $(V(C),C)$ belongs
to $B_2$.

\paragraph{Reducing a large component.}
Our main goal is to show that if the bags of any component $V(C)$
contain in total more than $m = \Theta(k^2 \ell^{4\eta+4})$ vertices of $G$, that is,
$|\X(V(C))| > m$, then 
one can, with a help of a number of oracle calls, reduce the graph $G$ by at least
one vertex. Fix such a component $C$.

Let $t_0 \in V(C)$ be the lowest node in $V(C)$ such that,
if $D$ is the set of nodes of $V(C)$ in the subtree of $T$ rooted in $t_0$,
then $|\X(D)| > m$.

Let $V_D = \X(D)$ and let $G_D = G[V_D \cup M]$.
Furthermore, let $S_D = \X(D \cap (B_2 \cup \{t_0\}))$; since
$|V(C) \cap B_2| \leq 2$ and the topmost vertex of $C$ belongs to $B_2$, 
we have $|D \cap (B_2 \cup \{t_0\})| \leq 2$ and hence $|S_D| \leq 2\eta+2$.
Since $T$ is a binary tree, the choice of $t_0$ ensures that 
$$|V_D| \leq 2m+\eta+1.$$
Note that $N_G(V_D \setminus S_D) \subseteq S_D \cup M$.
For a simple path $P$ in $G$, a \emph{traverse} of $P$ through $G_D$ is
a maximal subpath of $P$ with all internal vertices in $V_D \setminus S_D$.

\begin{lemma}\label{lem:neat}
If $(G,k)$ is a yes-instance to \kPath{}, then there exists
a simple path $P$ in $G$ with $k$ vertices that is either contained
in $V_D-S_D$ or whose every traverse through $G_D$ has at least one endpoint in $S_D$.
\end{lemma}
\begin{proof}
Let $P$ be a $k$-path in $G$ that contains maximum possible number of vertices
from $A_1$; we claim that $P$ satisfies the statement of the lemma.
Assume the contrary, let $Q$ be a traverse of $P$ through $G_D$ whose neither of the endpoints
belong to $S_D$. Since $P$ is not completely contained in $G_D-S_D$, and
$N_G(V_D \setminus S_D) \subseteq S_D \cup M$, we have that $Q$ is either a $(u,v,k')$-path
for some $u,v \in M$ and $1 \leq k' \leq k-2$ 
or a $(u,k')$-path for some $u \in M$ and $1 \leq k' \leq k-1$. 
Assume the first case; the proof for the second case is analogous.

Since $G_D-S_D$ does not contain any vertex of $A_2 \supseteq A_1$, from the maximality
of $\mathcal{P}_{u,v,k'}^0$ we infer that $\mathcal{P}_{u,v,k'} \subsetneq \mathcal{P}_{u,v,k'}^0$ (since it contains $Q$)
and, consequently, $|\mathcal{P}_{u,v,k'}| = k+1$. Thus, at least one $(u,v,k')$-path
$Q' \in \mathcal{P}_{u,v,k'}$ has no internal vertices on the $k$-path $P$. 
Consequently, by replacing $Q$ with $Q'$ on $P$, we obtain a simple $k$-path $P'$
with strictly more vertices of $A_1$ than $P$. This is a contradiction.
\cqed\end{proof}

A $k$-path as in the statement of Lemma~\ref{lem:neat} is henceforth called \emph{neat}.
Lemma~\ref{lem:neat} allows us to look only for a neat $k$-path in $G$.
Note that such a neat $k$-path $P$ contains at most $2|S_D| \leq 4\eta+4$ traverses of $G_D$: every
vertex of $S_D$ can be an endpoint of at most two traverses.

Let $P_1,\ldots,P_r$ be the traverses through $G_D$ of a neat $k$-path $P$.
For every $1 \leq i \leq r$, let $R_i$ be defined as the endpoints of $P_i$ that
lie in $M \cup S_D$. Let $k'$ be the total number of vertices
that lie on all paths $P_i$. Observe that 
the paths $(P_i)_{i=1}^r$ form a feasible solution to the \kLinkage{} instance
$\mathcal{I} := (G_D,k',S_D \cup M, (R_i)_{i=1}^r)$. On the other hand, 
if $(P_i')_{i=1}^r$ is any feasible solution to $\mathcal{I}$, then a path $P'$
obtained from $P$ by replacing every subpath $P_i$ with $P_i'$ is a neat $k$-path in $G$
as well.

Finally, note that there is only a bounded number of choices for the instance $\mathcal{I}$.
That is, either the sequence $(R_i)_{i=1}^r$ consists of a single empty set (if $P$ lives
entirely in $G_D-S_D$), or is a sequence of at most $4\eta+4$ requests, each containing one vertex
of $S_D$ and possibly a second vertex of $S_D \cup M$. Hence, the number of choices is bounded
by 
$$\rho := 1 + \sum_{j=0}^{4\eta+4} \left((2\eta+2) \cdot (\ell+2\eta+2)\right)^j = \Theta(\ell^{4\eta+4}).$$
For every choice of the sequence $(R_i)_{i=1}^r$ and every $0 \leq k' \leq k$, we invoke
the oracle on the \kLinkage{} instance $(G_D,k',(R_i)_{i=1}^r)$; recall that
$|V(G_D)| = |V_D| \leq 2m+\eta+1$.
In case of a positive answer, using self-reducibility of the \kLinkage{} problem
we find a feasible solution and mark all its vertices.
Let $A_3$ be the set of marked vertices for all choices of $k'$ and $(R_i)_{i=1}^r$.
The arguments so far allow us to delete $V_D \setminus (A_3 \cup S_D)$ from the graph $G$
without changing the answer to the \kPath{} problem on $(G,k)$.

It remains to argue that for the choice of $m$ we always delete at least one vertex.
Note that
$$|A_3| \leq \rho \cdot k \cdot k = \Oh(k^2 \ell^{4\eta+4})$$
and $|S_D| \leq 2\eta+2 = \Oh(1)$.
Thus, for sufficiently large $m = \Theta(k^2 \ell^{4\eta+4})$
we have that $V_D \setminus (A_3 \cup S_D)$ is nonempty, and we delete at one vertex.

\paragraph{Wrap up.}
Recall that we have shown a reduction rule that deletes at least one vertex of $G$
in the presence of a component $C$ whose bags contain
at least $m = \Theta(k^2 \ell^{4\eta+4})$ distinct vertices of $G$.
However, since $|B_2| \leq 2k(k+1)\ell^2$ and node of $T$ has at most two children,
there are at most $4k(k+1)\ell^2+1$ components. Consequently, if the reduction is not applicable,
      we have
$$|V(G)| = \Oh(k^4 \ell^{4\eta+6}).$$
Such an instance can be solved with a single call to \kLinkage{} with $k' = k$, $S = \emptyset$,
$r=1$, and $R_1 = \emptyset$.
This finishes the proof of Theorem~\ref{thm:eta-main2} and, consequently, of Theorem~\ref{thm:eta-main}.

